Direct numerical simulation of pattern formation in subaqueous sediment

We present results of direct numerical simulation of incompressible fluid flow over a thick bed of mobile, spherically-shaped particles. The algorithm is based upon the immersed boundary technique for fluid-solid coupling and uses a soft-sphere model for the solid-solid contact. Two parameter points in the laminar flow regime are chosen, leading to the emergence of sediment patterns classified as `small dunes', while one case under turbulent flow conditions leads to `vortex dunes' with significant flow separation on the lee side. Wavelength, amplitude and propagation speed of the patterns extracted from the spanwise-averaged fluid-bed interface are found to be consistent with available experimental data. The particle transport rates are well represented by available empirical models for flow over a plane sediment bed in both the laminar and the turbulent regimes.

==> additional_stuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%55
\section{additional material}
%============================================================
% table: numerical parameters
%
\begin{table}
  \begin{center}
\def~{\hphantom{0}}
  \begin{tabular}{lcccccccc}
      Case &
      $[\Lx \times \Ly \times \Lz]/\Dia$  & 
      $N_x \times N_y \times N_z$  &   
      $\hmean/\Delta x$ &
      $\Delta x^+$ &
      $\Dia/\Delta x$ & 
      \Npm &
      \Npf &
      channel \\[3pt]
      \caseLa &
      $307.2\times 76.8\times 12.8$ & 
      $3072\times 769\times 128$ & 
      267.70 & 
      0.12 &
      10 &
      ~75531 &
      ~3542 &
      closed\\
      %
      \caseLb &
      $307.2\times 76.8\times 12.8$ & 
      $3072\times 769\times 128$ & 
      265.33 &
      0.12 & 
      10 &
      ~75531 &
      ~3542 &
      closed\\
      \caseTa &
      $307.2\times 38.4\times 76.8$ & 
      $3072\times 385\times 768$ & 
      244.70 &
      1.07 & 
      10 &
      242160 &
      21252 &
      open\\
  \end{tabular}
  \caption{Numerical parameters of the sumulations.}
  \label{tab:numerical-parameters}
  \end{center}
\end{table}
%
% 
%============================================================
% figure: evolution of box kinetic energy
%
\begin{figure}
   \centering
       \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $\langle k \rangle_{xyz}/\ubulk^2$}
        \end{minipage}
        \begin{minipage}{.43\linewidth}
          %\centerline{$(b)$}
          \includegraphics[width=\linewidth]
          {../plots/Box_averaged_kinetic_energy_ALL.pdf}
          \centerline{\small
            $t\cdot \ubulk/\hmean$}
        \end{minipage}%\\[20pt]
        %
        \caption{
                 Time evolution of the box averaged 
                 turbulent kinetic 
                 energy.               
                 The simulation of case \caseTa\ was initially run
                 on a coarse grid while fixing the particles
                 in space (dashed-line in the plot).
                 The fully developed flow field was then refined to
                 the current grid resolution. 
                 Mobile particles
                 (except those at the bottom) were released first
                 at time $t=0$ thus insuring the flow field was
                 fully-developed (in the finer resolution)
                 when the particles were released ($t>0$).
                }
        \label{fig:time-evolution-of-kinetic-energy}
                                                                       
\end{figure}
%\clearpage
%
%============================================================
% figure: profiles of mean shear and velocity: L01 and T01
%
\begin{figure}
   \centering
        %
        \raisebox{15ex}{$(a)$}
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $(y-y_0)/\hmean$}
        \end{minipage}
        \begin{minipage}{.4\linewidth}
          %\centerline{$(a)$}
          \centerline{\mbox{}}
          \centerline{$\langle \tau \rangle /(\rho_f\ufric^2)$}
          \includegraphics[width=\linewidth]
          {../plots/Mean_Velocity_and_ShearProfile_laminar.pdf}
          \centerline{\small
            $\ufmean/\ubulk$}
        \end{minipage}
        %
        \hspace{2ex}
        \raisebox{15ex}{$(b)$}
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $(y-y_0)/\hmean$}
        \end{minipage}
        \begin{minipage}{.4\linewidth}
          %\centerline{$(b)$}
          \centerline{\mbox{}}
          \centerline{$\langle \tau \rangle /(\rho_f\ufric^2)$}
          \includegraphics[width=\linewidth]
          {../plots/Mean_Velocity_and_ShearProfile_turbulent.pdf}
          \centerline{\small
            $\ufmean/\ubulk$}
        \end{minipage}
        \caption{Wall-normal profiles of
                the mean streamwise fluid velocity (black) and
                total shear stress (blue).
                (\textit{a}), \caseLa; (\textit{b}) \caseTa.
                The total shear stress in case \caseTa is the sum
                of the viscous shear stress ({\color{blue}\dashed}) 
                and the Reynolds shear stress ({\color{blue}\chndot}). 
                The horizontal dashed lines show
                the offsets corresponding to the mean amplitude
                of the patterns ($\pm\hat{h}_{b,av}$). Friction
                velocity \ufric\ is determined by fitting a line
                to the linear region of $\langle \tau \rangle$ and
                extending it to $y_0$.
                }
        \label{fig:mean-velocity-and-shear-profile}
                                                                       
\end{figure}
%
%============================================================
% figure: evolution of particle flux
%
\begin{figure}
   \centering
       
         \raisebox{15ex}{$(b)$}
         \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $\partflowrate/\flowrateref$}
        \end{minipage}
        \begin{minipage}{.43\linewidth}
          %\centerline{$(b)$}
          \includegraphics[width=\linewidth]
          {../plots/ParticleFlux_time_evolution_All.pdf}
          \centerline{\small
            $t\cdot \ubulk/\hmean$}
        \end{minipage}\\[20pt]
        %
        \caption{
                 (\textit{b}) Time evolution of the particle
                  flux.
                }
        \label{fig:particle_flux_evolution}
                                                                       
\end{figure}
%
%============================================================
% figure: snapshot of the turbulent case z averaged slice
%
\begin{figure}
   \centering
        %
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $y/D$}
        \end{minipage}
        \begin{minipage}{.4\linewidth}
          %\centerline{$(a)$}
          \includegraphics[width=\linewidth]
          {../plots/slice_instant_ripple01Re3000_f0065_streamline.jpg}
          \centerline{\small
            $x/D$}
        \end{minipage}
        %
         \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $y/D$}
        \end{minipage}
         \begin{minipage}{0.4\linewidth}
          %\centerline{$(b)$}
          \includegraphics[width=\linewidth]
          {../plots/slice_zaveraged_ripple01Re3000_f0065_streamline.jpg}
          \centerline{\small
            $x/D$}
        \end{minipage}%\\[20pt]
        \caption{2D streamline plot in a closeup window for case T01.
                 (\textit{a}) for the data in figure
                 \ref{fig:instantaneous-snapshot-slice-instant-T01}.
                 (\textit{b}) for the data in figure
                 \ref{fig:instantaneous-snapshot-slice-zaveraged-T01}
                }
        \label{fig:streamline-plot-T01}
\end{figure}
%============================================================
% figure: snapshot of the turbulent case z averaged slice
%
\begin{figure}
   \centering
        %
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $y/D$}
        \end{minipage}
        \begin{minipage}{.7\linewidth}
          %\centerline{$(a)$}
          \includegraphics[width=\linewidth]
          {../plots/u_slice_instant_ripple01Re3000_f0065.jpg}
          %\centerline{\small
          %  $t\cdot u_b/h_f$;$\;t\cdot u_b/(2h_f)$}
        \end{minipage}\\[10pt]
        %
         \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $y/D$}
        \end{minipage}
         \begin{minipage}{0.7\linewidth}
          %\centerline{$(b)$}
          \includegraphics[width=\linewidth]
          {../plots/v_slice_instant_ripple01Re3000_f0065.jpg}
          \centerline{\small
            $x/D$}
        \end{minipage}%\\[20pt]
         \caption{(\textit{a})
                 Instantaneous snapshot of the
                 streamwise velocity in a plane located at 
                 $z=L_z/2$ for case T01. 
                 (\textit{b}) the same plot for wall-normal velocity}
        \label{fig:instantaneous-snapshot-slice-instant-T01}
\end{figure}
%
\begin{figure}
   \centering
        %
        \raisebox{7ex}{$(d)$} 
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $R_{\hbed^\prime\hbed^\prime}$}
        \end{minipage}
        \begin{minipage}{0.25\linewidth}
          %\centerline{(\textit{d})}
          \includegraphics[width=\linewidth]
          {../plots/Interface_correlation_selected_times_ripple01Re700.pdf}
          \centerline{\small $r_x/\Dia$ }
        \end{minipage}%\\[10pt]
        %
        \hspace{1ex}
        \raisebox{7ex}{$(e)$} 
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $R_{\hbed^\prime\hbed^\prime}$}
        \end{minipage}
        \begin{minipage}{0.25\linewidth}
         % \centerline{(\textit{e})}
          \includegraphics[width=\linewidth]
          {../plots/Interface_correlation_selected_times_ripple03Re700.pdf}
          \centerline{\small $r_x/\Dia$}
        \end{minipage}%\\[10pt]
        %
        \hspace{1ex}
        \raisebox{7ex}{$(f)$} 
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $R_{\hbed^\prime\hbed^\prime}$}
        \end{minipage}
        \begin{minipage}{0.25\linewidth}
         % \centerline{(\textit{f})}
          \includegraphics[width=\linewidth]
          {../plots/Interface_correlation_selected_times_ripple01Re3000.pdf}
          \centerline{\small $r_x/\Dia$}
        \end{minipage}\\
         %
        \raisebox{12ex}{$(c)$} 
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $\hat{h}_b/\Dia$}
        \end{minipage}
        \begin{minipage}{0.4\linewidth}
          %\centerline{(\textit{a})}
          \includegraphics[width=\linewidth]
        {../plots/Interface_dominant_amplitude_evolution_All.pdf}     
          \centerline{\small $t\cdot \ubulk/\hmean$ }
        \end{minipage}
        %
        \hspace{1pt}
        \raisebox{12ex}{$(d)$} 
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
        \end{minipage}
        \begin{minipage}{0.4\linewidth}
          %\centerline{(\textit{a})}
          \includegraphics[width=\linewidth]
        {../plots/Interface_dominant_phase_angle_evolution_All.pdf}     
          \centerline{\small $t\cdot \ubulk/\hmean$ }
        \end{minipage}
\end{figure}
%============================================================
% figure: slice snapshots of the turbulent case
%
\begin{figure}
   \centering
        %
        \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $y/D$}
        \end{minipage}
        \begin{minipage}{.7\linewidth}
          %\centerline{$(a)$}
          \includegraphics[width=\linewidth]
          {../plots/u_slice_zaveraged_ripple01Re3000_f0065.jpg}
          %\centerline{\small
          %  $t\cdot u_b/h_f$;$\;t\cdot u_b/(2h_f)$}
        \end{minipage}\\[10pt]
        %
         \begin{minipage}{2ex}
          \rotatebox{90}
          {\small $y/D$}
        \end{minipage}
         \begin{minipage}{0.7\linewidth}
          %\centerline{$(b)$}
          \includegraphics[width=\linewidth]
          {../plots/v_slice_zaveraged_ripple01Re3000_f0065.jpg}
          \centerline{\small
            $x/D$}
        \end{minipage}%\\[20pt]
        \caption{(\textit{a})
                 Instantaneous snapshot of a spanwise-averaged
                 streamwise velocity for case T01. 
                 (\textit{b}) the same plot for wall-normal velocity}
        \label{fig:instantaneous-snapshot-slice-zaveraged-T01}
\end{figure}
%\clearpage
%
%\clearpage
%
%% %============================================================
%% % figure: slice snapshots of the turbulent case
%% %
%% \begin{figure}
%%    \centering
%%          %
%%          \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $y/D$}
%%         \end{minipage}
%%          \begin{minipage}{0.5\linewidth}
%%           \centerline{$(a)$}
%%           \includegraphics[width=\linewidth]
%%           {../plots/u_slice_zaveraged_ripple01Re700_f0127.jpg}
%%           \centerline{\small $x/D$}
%%         \end{minipage}\\[10pt]
%%          %
%%          \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $y/D$}
%%         \end{minipage}
%%          \begin{minipage}{0.5\linewidth}
%%           \centerline{$(b)$}
%%           \includegraphics[width=\linewidth]
%%           {../plots/v_slice_zaveraged_ripple01Re700_f0127.jpg}
%%           \centerline{\small $x/D$}
%%         \end{minipage}%\\[20pt]
%%         \caption{(\textit{a})
%%                  Instantaneous snapshot of a spanwise-averaged
%%                  streamwise velocity for case L01. 
%%                  (\textit{b}) the same plot for wall-normal velocity}
%%         \label{fig:instantaneous-snapshot-slice-zaveraged-L01}
%% \end{figure}
%% %
%% %============================================================
%% % figure: snapshot of the turbulent case z averaged slice
%% %
%% \begin{figure}
%%    \centering
%%          %
%%          \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $y/D$}
%%          \end{minipage}
%%          \begin{minipage}{0.5\linewidth}
%%           %\centerline{$(b)$}
%%           \includegraphics[width=\linewidth]
%%           {../plots/slice_zaveraged_ripple01Re700_f0127_streamline.jpg}
%%           \centerline{\small
%%             $x/D$}
%%         \end{minipage}%\\[20pt]
%%         \caption{2D streamline plot in a closeup window for case L01.
%%                  corresponding to the data in figure
%%                  \ref{fig:instantaneous-snapshot-slice-zaveraged-L01}.
%%                 }
%%         \label{fig:streamline-plot-T01}
%% \end{figure}


%% %% \begin{figure}
%%         \centering
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{a})}
%%           \includegraphics[width=\linewidth]
%%         {../plots/Interface_dominant_amplitudes_evolution_ripple01Re700.pdf}     
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%         %
%%         %\hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{b})}
%%           \includegraphics[width=\linewidth]
%%          {../plots/Interface_dominant_amplitudes_evolution_ripple03Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$ }
%%         \end{minipage}
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{c})}
%%           \includegraphics[width=\linewidth]
%%         {../plots/Interface_dominant_amplitudes_evolution_ripple01Re3000.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}\\[10pt]
%%         %%
%%         %%
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{d})}
%%           \includegraphics[width=\linewidth]
%%         {../plots/Interface_dominant_phase_angle_speed_ripple01Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$ }
%%         \end{minipage}
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%          {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{e})}
%%           \includegraphics[width=\linewidth]
%%         {../plots/Interface_dominant_phase_angle_speed_ripple03Re700.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{f})}
%%           \includegraphics[width=\linewidth]
%%         {../plots/Interface_dominant_phase_angle_speed_ripple01Re3000.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         %
%%         \caption{(\textit{a,c,e})
%%                  Time evolution of the
%%                  amplitude spectral density corresponding to the 
%%                  bed-fluid interface $\hbed^\prime$ (time instants shifted at 
%%                  certain offset
%%                  in the vertical axis for clarity).
%%                  (\textit{b,d,f})
%%                  Time evolution of the amplitude of the 
%%                  first five modes corresponding to wavelengths
%%                  $\lambda_x=\Lx$ ({\color{blue}\solidthick});
%%                  $\lambda_x=\Lx/2$ ({\color{red}\solidthick});
%%                  $\lambda_x=\Lx/3$ ({\color{black}\solidthick});
%%                  $\lambda_x=\Lx/4$ ({\color{magenta}\solidthick});
%%                  $\lambda_x=\Lx/5$ ({\color{green}\solidthick}).
%%                  Plots (\textit{a,b}) correspond to case \caseLa,
%%                   (\textit{c,d}) to case \caseLb and
%%                   (\textit{e,f}) to case \caseTa
%%               }
%%    \label{fig:interface_space_time}
%% \end{figure}
%\clearpage
%% %
%% %============================================================
%% % figure: particle bed correlation grayscale 
%% %
%% \begin{figure}
%%         \centering
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{a})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_correlation_space_time_ripple01Re700.jpg}
%%           \centerline{\small $r_x/\Dia$ }
%%         \end{minipage}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{b})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_correlation_space_time_ripple03Re700.jpg}
%%           \centerline{\small $r_x/\Dia$ }
%%         \end{minipage}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{c})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_correlation_space_time_ripple01Re3000.jpg}
%%           \centerline{\small $r_x/\Dia$ }
%%         \end{minipage}
%%         %
%%         \caption{Time evolution of the auto-correlation coefficient
%%                  $R_{\hbed'\hbed'}$ of the fluid-bed interface $\hbed^\prime$ as
%%                  a  function  of streamwise separation $r_x$ which
%%                  is an indirect measure of the mean wavelength of 
%%                  the fluid-bed interface.
%%                  (\textit{a}),~\caseLa;   
%%                  (\textit{b}),~\caseLb; 
%%                  (\textit{c}),~\caseTa; 
%%                  %Note that mean wavelength $\lambda_{av}> \Lx/2$
%%                  %will not be represented by this plot.            
%%                 }
%%    \label{fig:auto-correlation-of-fluid-bed-interface}
%% \end{figure}
%% \clearpage
%% %
%% %============================================================
%% % figure: 
%% %
%% \begin{figure}
%%         \centering
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $R_{\hbed^\prime\hbed^\prime}$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{a})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_correlation_selected_times_ripple01Re700.pdf}
%%           \centerline{\small $r_x/\Dia$ }
%%         \end{minipage}%\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $R_{\hbed^\prime\hbed^\prime}$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{b})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_correlation_selected_times_ripple03Re700.pdf}
%%           \centerline{\small $r_x/\Dia$}
%%         \end{minipage}%\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $R_{\hbed^\prime\hbed^\prime}$}
%%         \end{minipage}
%%         \begin{minipage}{0.3\linewidth}
%%           \centerline{(\textit{c})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_correlation_selected_times_ripple01Re3000.pdf}
%%           \centerline{\small $r_x/\Dia$}
%%         \end{minipage}
%%         %
%%         \caption{\AGK{The same data as in figure
%%                   \ref{fig:auto-correlation-of-fluid-bed-interface}
%%                   plotted differently for our choice. To highlight
%%                   amplitude of the signal, all the curves are
%%                   normalized by $R(r_x=0)$ of last the curve,
%%                   otherwise all plots will have $R=1$ at $r_x=0$}
%%                  (\textit{a}),~\caseLa;
%%                  (\textit{b}),~\caseLb;
%%                   (\textit{c}),~\caseTa.
%%                   Color coding: blue,$t=0$; red,$t=t_{last}$.
%%                   Plots are at certain time interval 
%%               }
%%    \label{fig:auto-correlation-of-fluid-bed-interface2}
%% \end{figure}
%% \clearpage
%% %
%============================================================
% figure: 
%
%% \begin{figure}
%%         \centering
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{a})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_spectra_ripple01Re700.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%          \hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{b})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_amplitudes_evolution_ripple01Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$ }
%%         \end{minipage}\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{c})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_spectra_ripple03Re700.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%          \hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{d})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_amplitudes_evolution_ripple03Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$ }
%%         \end{minipage}\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{e})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_spectra_ripple01Re3000.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%          \hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\hat{h}_b/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{f})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_amplitudes_evolution_ripple01Re3000.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         %
%%         \caption{(\textit{a,c,e})
%%                  Time evolution of the
%%                  amplitude spectral density corresponding to the 
%%                  bed-fluid interface $\hbed^\prime$ (time instants shifted at 
%%                  certain offset
%%                  in the vertical axis for clarity).
%%                  (\textit{b,d,f})
%%                  Time evolution of the amplitude of the 
%%                  first five modes corresponding to wavelengths
%%                  $\lambda_x=\Lx$ ({\color{blue}\solidthick});
%%                  $\lambda_x=\Lx/2$ ({\color{red}\solidthick});
%%                  $\lambda_x=\Lx/3$ ({\color{black}\solidthick});
%%                  $\lambda_x=\Lx/4$ ({\color{magenta}\solidthick});
%%                  $\lambda_x=\Lx/5$ ({\color{green}\solidthick}).
%%                  Plots (\textit{a,b}) correspond to case \caseLa,
%%                   (\textit{c,d}) to case \caseLb and
%%                   (\textit{e,f}) to case \caseTa
%%               }
%%    \label{fig:interface_space_time}
%% \end{figure}
%% \clearpage
%% %
%% %
%% %============================================================
%% % figure: 
%% %
%% \begin{figure}
%%         \centering
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\varphi/(2\pi)\cdot \lambda_x/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{a})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_phase_spectra_ripple01Re700.pdf}
%%           \centerline{\small $\lambda_x/D$ }
%%         \end{minipage}
%%          \hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\varphi/(2\pi)\cdot \lambda_x/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{b})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_phase_angle_evolution_ripple01Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$ }
%%         \end{minipage}\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\varphi/(2\pi)\cdot \lambda_x/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{c})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_phase_spectra_ripple03Re700.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%          \hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\varphi/(2\pi)\cdot \lambda_x/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{d})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_phase_angle_evolution_ripple03Re700.pdf}
%%           \centerline{\small $t\cdot  \ubulk/\hmean$ }
%%         \end{minipage}\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\varphi/(2\pi)\cdot \lambda_x/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{e})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_phase_spectra_ripple01Re3000.pdf}
%%           \centerline{\small $\lambda_x/\Dia$ }
%%         \end{minipage}
%%          \hspace{10pt}
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $\varphi/(2\pi)\cdot \lambda_x/\Dia$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{f})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_phase_angle_evolution_ripple01Re3000.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         %
%%         \caption{(\textit{a,c,e})
%%                  Time evolution of the
%%                  phase angle spectral density corresponding to the 
%%                  bed-fluid interface.
%%                  (\textit{b,d,f})
%%                  Time evolution of the phase angle of the 
%%                  first five modes corresponding to wavelengths
%%                  $\lambda_x=\Lx$ ({\color{blue}\solidthick});
%%                  $\lambda_x=\Lx/2$ ({\color{red}\solidthick});
%%                  $\lambda_x=\Lx/3$ ({\color{black}\solidthick});
%%                  $\lambda_x=\Lx/4$ ({\color{magenta}\solidthick});
%%                  $\lambda_x=\Lx/5$ ({\color{green}\solidthick}).
%%                  Plots (\textit{a,b}) correspond to \caseLa,
%%                   (\textit{c,d}) to \caseLb and
%%                   (\textit{e,f}) to case \caseTa
%%               }
%%    \label{fig:interface_space_time}
%% \end{figure}
%% \clearpage
%% %
%% %============================================================
%% % figure: 
%% %
%% \begin{figure}
%%         \centering
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{a})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_phase_angle_speed_ripple01Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$ }
%%         \end{minipage}\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{b})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_phase_angle_speed_ripple03Re700.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}\\[10pt]
%%         %
%%         \begin{minipage}{2ex}
%%           \rotatebox{90}
%%           {\small $d\varphi/dt\cdot(\lambda_x/2\pi)/\ubulk$}
%%         \end{minipage}
%%         \begin{minipage}{0.45\linewidth}
%%           \centerline{(\textit{c})}
%%           \includegraphics[width=\linewidth]
%%           {../plots/Interface_dominant_phase_angle_speed_ripple01Re3000.pdf}
%%           \centerline{\small $t\cdot \ubulk/\hmean$}
%%         \end{minipage}
%%         %
%%         \caption{Phase speed as a function of time of the 
%%                  first five modes corresponding to wavelengths
%%                  $\lambda_x=\Lx$ ({\color{blue}\solidthick});
%%                  $\lambda_x=\Lx/2$ ({\color{red}\solidthick});
%%                  $\lambda_x=\Lx/3$ ({\color{black}\solidthick});
%%                  $\lambda_x=\Lx/4$ ({\color{magenta}\solidthick});
%%                  $\lambda_x=\Lx/5$ ({\color{green}\solidthick}).
%%                  (\textit{a}),~\caseLa;
%%                  (\textit{b}),~\caseLb;
%%                   (\textit{c}),~\caseTa.
%%               }
%%    \label{fig:interface_phase_speed}
%% \end{figure}
%% \clearpage
%% %


